Can Domains Be Transferred Across Languages in Multi-Domain Multilingual Neural Machine Translation?

Previous works mostly focus on either multilingual or multi-domain aspects of neural machine translation (NMT). This paper investigates whether the domain information can be transferred across languages on the composition of multi-domain and multilingual NMT, particularly for the incomplete data condition where in-domain bitext is missing for some language pairs. Our results in the curated leave-one-domain-out experiments show that multi-domain multilingual (MDML) NMT can boost zero-shot translation performance up to +10 gains on BLEU, as well as aid the generalisation of multi-domain NMT to the missing domain. We also explore strategies for effective integration of multilingual and multi-domain NMT, including language and domain tag combination and auxiliary task training. We find that learning domain-aware representations and adding target-language tags to the encoder leads to effective MDML-NMT.

==> tab-all-md.tex <==
\begin{table}[]
\begin{tabular}{llllllllllllllllllllllllllll}
     &            &       &       &       &         &           &       &       &       &         &           &       &       &       &         &           &         &       &       &         &           &           &       &       &         &           &     \\
     &            & LAW   &       &       &         &           & IT    &       &       &         &           & KORAN &       &       &         &           & Medical &       &       &         &           & SUBTITLES &       &       &         &           & avg \\
     &            & LAW   & IT    & KORAN & MEDICAL & SUBTITLES & LAW   & IT    & KORAN & MEDICAL & SUBTITLES & LAW   & IT    & KORAN & MEDICAL & SUBTITLES & LAW     & IT    & KORAN & MEDICAL & SUBTITLES & LAW       & IT    & KORAN & MEDICAL & SUBTITLES &     \\
denc & md         & 10.52 & 34.53 & 15.84 & 49.31   & 20.89     & 39.69 & 20.37 & 15.75 & 49.16   & 21.29     &       &       &       &         &           & 39.71   & 34.05 & 16.44 & 19.46   & 18.82     &           &       &       &         &           &     \\
     & md-disc    & 10.62 & 34.59 & 16.66 & 48.75   & 19.36     & 39.92 & 19.43 & 16.51 & 49.29   & 20.38     &       &       &       &         &           & 40.43   & 34.16 & 17.14 & 20.79   & 19.64     &           &       &       &         &           &     \\
     & md-aware   & 10.37 & 35.46 & 17.38 & 49.58   & 20.38     & 40.58 & 21.70 & 17.07 & 49.39   & 21.30     &       &       &       &         &           & 40.00   & 34.15 & 17.94 & 20.07   & 19.32     &           &       &       &         &           &     \\
ddec & md         & 9.21  & 35.67 & 16.65 & 49.06   & 18.18     & 38.56 & 12.39 & 16.04 & 49.29   & 20.58     &       &       &       &         &           & 38.12   & 33.69 & 15.69 & 19.56   & 18.45     &           &       &       &         &           &     \\
     & md-disc    & 9.78  & 33.63 & 16.80 & 48.77   & 18.25     & 39.68 & 11.01 & 15.78 & 48.41   & 18.36     &       &       &       &         &           & 39.55   & 33.88 & 16.65 & 18.03   & 19.01     &           &       &       &         &           &     \\
     & md-aware   & 9.51  & 34.17 & 17.62 & 49.39   & 18.95     & 39.72 & 12.25 & 15.39 & 49.80   & 19.85     &       &       &       &         &           & 39.20   & 33.55 & 17.81 & 18.46   & 19.32     &           &       &       &         &           &     \\
0    & mdml       & 10.89 & 30.33 & 11.24 & 40.28   & 14.40     & 34.18 & 22.14 & 12.35 & 45.24   & 16.02     & 36.55 & 34.30 & 8.74  & 45.41   & 17.64     & 36.02   & 32.86 & 11.79 & 22.02   & 16.72     & 36.75     & 34.53 & 12.54 & 45.72   & 7.28      &     \\
     & mdml-adv   & 11.92 & 32.83 & 12.00 & 44.83   & 15.89     & 35.83 & 22.67 & 12.63 & 45.51   & 16.69     & 36.10 & 34.15 & 9.13  & 45.85   & 17.25     & 36.54   & 33.38 & 12.61 & 22.19   & 16.70     & 36.33     & 33.06 & 13.52 & 45.46   & 8.64      &     \\
     & mdml-aware & 12.12 & 34.25 & 13.19 & 45.50   & 17.08     & 36.19 & 23.60 & 12.50 & 45.31   & 16.46     & 37.59 & 34.94 & 9.53  & 46.61   & 18.35     & 36.40   & 33.41 & 12.58 & 21.49   & 16.70     & 37.28     & 34.25 & 13.77 & 45.91   & 9.21      &     \\
1    & mdml       & 11.98 & 32.83 & 11.74 & 44.16   & 15.56     & 34.45 & 22.64 & 12.13 & 44.77   & 3.99      & 36.37 & 34.18 & 8.08  & 45.79   & 17.54     & 33.54   & 31.28 & 11.39 & 21.05   & 15.79     & 36.36     & 33.24 & 12.18 & 45.39   & 8.63      &     \\
     & mdml-adv   & 12.11 & 33.40 & 13.15 & 45.68   & 16.37     & 36.41 & 23.43 & 12.69 & 45.44   & 16.62     & 36.85 & 33.41 & 9.26  & 45.77   & 17.96     & 36.55   & 33.32 & 12.83 & 21.59   & 16.95     & 36.31     & 33.14 & 12.63 & 45.73   & 8.16      &     \\
     & mdml-aware & 11.82 & 33.70 & 13.19 & 45.44   & 16.59     & 36.58 & 23.07 & 12.39 & 45.65   & 16.87     & 37.16 & 34.44 & 9.08  & 45.82   & 17.48     & 36.87   & 33.41 & 12.98 & 21.54   & 16.74     & 37.35     & 33.88 & 13.89 & 46.24   & 9.51      &     \\
2    & mdml       & 9.39  & 34.08 & 12.24 & 45.49   & 17.20     & 34.72 & 21.29 & 12.28 & 44.86   & 4.48      & 37.48 & 35.13 & 8.28  & 46.11   & 18.29     & 36.26   & 34.08 & 11.83 & 22.06   & 17.53     & 37.04     & 34.25 & 12.04 & 45.85   & 9.54      &     \\
     & mdml-adv   & 10.84 & 33.90 & 13.05 & 45.36   & 16.81     & 35.88 & 22.92 & 12.31 & 44.84   & 17.19     & 37.79 & 35.24 & 8.45  & 46.54   & 18.70     & 36.49   & 33.67 & 12.82 & 22.27   & 17.07     & 37.01     & 33.89 & 13.10 & 45.99   & 9.10      &     \\
     & mdml-aware &  12.29 & 34.50 & 12.50 & 45.54   & 16.61     & 36.11 & 22.70 & 12.54 & 45.46   & 16.77     & 37.89 & 34.93 & 8.39  & 46.30   & 19.02     & 36.77   & 34.06 & 12.81 & 22.62   & 17.21     & 37.62     & 34.46 & 13.35 & 46.05   & 10.75     &     \\
3    & mdml       & 13.14 & 33.95 & 12.53 & 45.57   & 16.51     & 34.37 & 20.63 & 12.17 & 44.85   & 3.64      & 37.62 & 34.40 & 8.01  & 45.59   & 18.05     & 36.63   & 33.72 & 12.26 & 21.13   & 16.79     & 37.21     & 34.09 & 12.88 & 45.95   & 5.21      &     \\
     & mdml-adv   & 11.81 & 33.16 & 12.40 & 45.03   & 15.36     & 36.46 & 19.47 & 12.80 & 45.15   & 16.80     & 36.95 & 33.82 & 8.90  & 45.94   & 17.67     & 36.50   & 33.43 & 12.92 & 21.97   & 16.58     & 36.35     & 33.25 & 13.23 & 45.87   & 5.78      &     \\
     & mdml-aware & 11.47 & 34.15 & 13.08 & 45.70   & 16.94     & 36.69 & 17.91 & 12.98 & 45.93   & 16.76     & 37.90 & 34.31 & 8.65  & 46.37   & 18.80     & 37.26   & 34.01 & 12.98 & 19.75   & 16.95     & 37.50     & 33.94 & 13.89 & 46.13   & 6.34      &     \\
4    & mdml       &  10.57  & 33.88 & 12.71 & 45.84   & 17.26     & 34.78 & 18.32 & 12.77 & 45.17   & 16.34     & 36.85 & 34.41 & 6.87  & 45.06   & 17.98     & 35.68   & 33.39 & 12.06 & 20.04   & 17.07     & 36.71     & 34.13 & 12.54 & 45.68   & 10.25     &     \\
     & mdml-adv   & 11.36 & 33.63 & 13.13 & 45.57   & 16.91     & 36.73 & 22.69 & 12.80 & 45.44   & 17.28     & 36.58 & 32.10 & 7.13  & 45.56   & 17.25     & 35.77   & 33.30 & 12.50 & 20.88   & 16.60     & 36.67     & 33.83 & 12.87 & 45.72   & 9.44      &     \\
     & mdml-aware & 11.25 & 31.78 & 11.85 & 43.17   & 15.30     & 37.04 & 21.94 & 12.50 & 45.70   & 17.45     & 37.82 & 34.95 & 8.73  & 46.33   & 18.48     & 36.91   & 33.97 & 12.79 & 20.69   & 17.23     & 35.70     & 33.34 & 12.28 & 44.73   & 10.34     &     \\
5    & mdml       & 5.21  & 25.27 & 11.73 & 41.75   & 13.23     & 34.38 & 17.56 & 11.25 & 43.36   & 15.33     & 34.31 & 25.24 & 4.53  & 41.87   & 13.68     & 33.01   & 22.80 & 11.99 & 9.12    & 12.47     & 34.04     & 24.45 & 12.47 & 41.00   & 4.36      &     \\
     & mdml-adv   & 2.25  & 22.54 & 13.93 & 40.77   & 13.13     & 33.02 & 17.47 & 12.07 & 40.63   & 13.36     & 35.37 & 31.91 & 4.89  & 44.16   & 15.51     & 33.22   & 28.73 & 11.72 & 12.41   & 11.55     & 35.91     & 31.34 & 11.91 & 44.31   & 5.18      &     \\
     & mdml-aware & 3.37  & 26.05 & 13.72 & 40.20   & 13.02     & 32.03 & 18.85 & 13.13 & 39.21   & 10.46     & 35.82 & 32.24 & 4.23  & 45.98   & 15.94     & 32.99   & 29.81 & 11.35 & 9.35    & 13.41     & 34.36     & 23.59 & 11.80 & 44.62   & 4.14      &    
\end{tabular}
\end{table}

==> tab-moe.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llrrrrr|r}
\toprule
              & model      & \textsc{Law} & \textsc{IT} & \textsc{Kor} & \textsc{Med} & \textsc{Sub} & AVG \\
\midrule
\midrule
% D-ENC & multi-domain & \\
% D-DEC & multi-domain & \\
% \midrule
\multicolumn{2}{c}{Adapter-based}& \\
\midrule
\multirow{3}{*}{\tenc}       & MDML       & \\
 & +adv   \\
                             & +aware & \underline{31.56}                    \\

\midrule
\multirow{3}{*}{\shortstack[l]{\tenc\\ \denc}} & MDML       &      \\
                             & +adv   & 26.09                   &  \\
                             & +aware &   \\
\midrule
\multirow{3}{*}{\shortstack[l]{\tenc\\ \ddec}} & MDML       &  \\
                             & +adv   &   \\
                             & +aware & \\
\midrule
\midrule
\multirow{3}{*}{\tdec}       & MDML       & \\

     & +adv   & \\
                             & +aware & \\
\midrule
\multirow{3}{*}{\shortstack[l]{\tdec\\ \denc}} & MDML       & \\
                             & +adv   & \\
                             & +aware &  \\
\midrule
\multirow{3}{*}{\shortstack[l]{\tdec\\ \ddec}} & MDML       &  \\
                             & +adv   & \\
                             & +aware &  \\
\bottomrule
\end{tabular}}
\caption{Average BLEU score of Mixture-of-Expert models (32 experts) on each domain in leave-one-out \textsc{Law} domain. }
\label{tab:moe}
\end{center}
\vspace{-5mm}
\end{table}
